Python bindings for libcloudph++

This technical note introduces the Python bindings for libcloudph++. The libcloudph++ is a C++ library of algorithms for representing atmospheric cloud microphysics in numerical models. The bindings expose the complete functionality of the library to the Python users. The bindings are implemented using the Boost.Python C++ library and use NumPy arrays. This note includes listings with Python scripts exemplifying the use of selected library components. An example solution for using the Python bindings to access libcloudph++ from Fortran is presented.

==> lst/api_common.py.tex <==
\begin{Verbatim}[commandchars=\\\{\}]
\PY{k+kn}{import} \PY{n+nn}{sys}
\PY{n}{sys}\PY{o}{.}\PY{n}{path}\PY{o}{.}\PY{n}{insert}\PY{p}{(}\PY{l+m+mi}{0}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{../../bindings/python/}\PY{l+s}{\PYZdq{}}\PY{p}{)}

\PY{c}{\PYZsh{}\PYZlt{}listing\PYZhy{}1\PYZgt{}}
\PY{k+kn}{from} \PY{n+nn}{libcloudphxx} \PY{k+kn}{import} \PY{n}{common}\PY{p}{,} \PY{n}{git\PYZus{}revision}

\PY{k}{print} \PY{n}{git\PYZus{}revision}

\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{common.p\PYZus{}vs(273.16)=}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{p\PYZus{}vs}\PY{p}{(}\PY{l+m+mf}{273.16}\PY{p}{)}
\PY{k}{assert} \PY{n+nb}{abs}\PY{p}{(}\PY{n}{common}\PY{o}{.}\PY{n}{p\PYZus{}vs}\PY{p}{(}\PY{l+m+mf}{273.16}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{l+m+mf}{611.73}\PY{p}{)} \PY{o}{\PYZlt{}} \PY{o}{.}\PY{l+m+mo}{001}
\PY{c}{\PYZsh{}\PYZlt{}/listing\PYZhy{}1\PYZgt{}}

\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{R\PYZus{}d =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{R\PYZus{}d}
\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{c\PYZus{}pd =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{c\PYZus{}pd}
\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{g =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{g}
\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{p\PYZus{}1000 =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{p\PYZus{}1000}
\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{eps =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{eps}
\PY{k}{print} \PY{l+s}{\PYZdq{}}\PY{l+s}{rho\PYZus{}w =}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{common}\PY{o}{.}\PY{n}{rho\PYZus{}w}

\PY{n}{th} \PY{o}{=} \PY{l+m+mi}{300}
\PY{n}{rv} \PY{o}{=} \PY{o}{.}\PY{l+m+mo}{01}

\PY{k}{print} \PY{n}{common}\PY{o}{.}\PY{n}{th\PYZus{}dry2std}\PY{p}{(}\PY{n}{th}\PY{p}{,} \PY{n}{rv}\PY{p}{)}	
\PY{k}{assert} \PY{n}{common}\PY{o}{.}\PY{n}{th\PYZus{}std2dry}\PY{p}{(}\PY{n}{common}\PY{o}{.}\PY{n}{th\PYZus{}dry2std}\PY{p}{(}\PY{n}{th}\PY{p}{,} \PY{n}{rv}\PY{p}{)}\PY{p}{,} \PY{n}{rv}\PY{p}{)} \PY{o}{==} \PY{n}{th}

\PY{n}{rd3} \PY{o}{=} \PY{p}{(}\PY{o}{.}\PY{l+m+mf}{2e\PYZhy{}6}\PY{p}{)}\PY{o}{*}\PY{o}{*}\PY{l+m+mi}{3}
\PY{k}{assert} \PY{n}{common}\PY{o}{.}\PY{n}{rw3\PYZus{}cr}\PY{p}{(}\PY{n}{rd3}\PY{p}{,} \PY{o}{.}\PY{l+m+mi}{5}\PY{p}{,} \PY{l+m+mi}{300}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{n}{rd3}
\PY{k}{assert} \PY{n}{common}\PY{o}{.}\PY{n}{S\PYZus{}cr}\PY{p}{(}\PY{n}{rd3}\PY{p}{,} \PY{o}{.}\PY{l+m+mi}{5}\PY{p}{,} \PY{l+m+mi}{300}\PY{p}{)} \PY{o}{\PYZgt{}} \PY{l+m+mi}{1}
\end{Verbatim}


==> lst/const_cp.hpp.tex <==
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{pragma once}

\PY{c+cp}{\PYZsh{}}\PY{c+cp}{include \PYZlt{}libcloudph++}\PY{c+cp}{/}\PY{c+cp}{common}\PY{c+cp}{/}\PY{c+cp}{units.hpp\PYZgt{} }\PY{c+c1}{// TODO: do detail?}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{include \PYZlt{}libcloudph++}\PY{c+cp}{/}\PY{c+cp}{common}\PY{c+cp}{/}\PY{c+cp}{macros.hpp\PYZgt{} }\PY{c+c1}{// TODO: do detail?}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{include \PYZlt{}libcloudph++}\PY{c+cp}{/}\PY{c+cp}{common}\PY{c+cp}{/}\PY{c+cp}{moist\PYZus{}air.hpp\PYZgt{}}

\PY{k}{namespace} \PY{n}{libcloudphxx}
\PY{p}{\PYZob{}}
  \PY{k}{namespace} \PY{n}{common}
  \PY{p}{\PYZob{}}
    \PY{k}{namespace} \PY{n}{const\PYZus{}cp}
    \PY{p}{\PYZob{}}
      \PY{k}{using} \PY{n}{moist\PYZus{}air}\PY{o}{:}\PY{o}{:}\PY{n}{c\PYZus{}pw}\PY{p}{;}
      \PY{k}{using} \PY{n}{moist\PYZus{}air}\PY{o}{:}\PY{o}{:}\PY{n}{c\PYZus{}pv}\PY{p}{;}
      \PY{k}{using} \PY{n}{moist\PYZus{}air}\PY{o}{:}\PY{o}{:}\PY{n}{R\PYZus{}v}\PY{p}{;}
      \PY{k}{using} \PY{n}{moist\PYZus{}air}\PY{o}{:}\PY{o}{:}\PY{n}{eps}\PY{p}{;}
      \PY{k}{typedef} \PY{n}{divide\PYZus{}typeof\PYZus{}helper}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{energy}\PY{p}{,} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{mass}\PY{o}{\PYZgt{}}\PY{o}{:}\PY{o}{:}\PY{n}{type} \PY{n}{energy\PYZus{}over\PYZus{}mass}\PY{p}{;}


      \PY{c+c1}{// water triple point parameters}
      \PY{n}{libcloudphxx\PYZus{}const}\PY{p}{(}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{pressure}\PY{p}{,} \PY{n}{p\PYZus{}tri}\PY{p}{,} \PY{l+m+mf}{611.73}\PY{p}{,} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{pascals}\PY{p}{)} \PY{c+c1}{// pressure}
      \PY{n}{libcloudphxx\PYZus{}const}\PY{p}{(}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{temperature}\PY{p}{,} \PY{n}{T\PYZus{}tri}\PY{p}{,} \PY{l+m+mf}{273.16}\PY{p}{,} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{kelvins}\PY{p}{)} \PY{c+c1}{// temperature}
      \PY{n}{libcloudphxx\PYZus{}const}\PY{p}{(}\PY{n}{energy\PYZus{}over\PYZus{}mass}\PY{p}{,} \PY{n}{l\PYZus{}tri}\PY{p}{,} \PY{l+m+mf}{2.5e6}\PY{p}{,} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{joules} \PY{o}{/} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{kilograms}\PY{p}{)} \PY{c+c1}{// latent heat of evaporation}

      \PY{c+c1}{// saturation vapour pressure for water assuming constant c\PYZus{}p\PYZus{}v and c\PYZus{}p\PYZus{}w}
      \PY{c+c1}{// with constants taken at triple point}
      \PY{c+c1}{// (solution to the Clausius\PYZhy{}Clapeyron equation assuming rho\PYZus{}vapour \PYZlt{}\PYZlt{} rho\PYZus{}liquid)}
\PY{c+c1}{//\PYZlt{}listing\PYZhy{}1\PYZgt{}}
      \PY{k}{template} \PY{o}{\PYZlt{}}\PY{k}{typename} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}
      \PY{n}{BOOST\PYZus{}GPU\PYZus{}ENABLED}
      \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{pressure}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{n}{p\PYZus{}vs}\PY{p}{(}
        \PY{k}{const} \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{temperature}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{o}{\PYZam{}}\PY{n}{T}
      \PY{p}{)} 
\PY{c+c1}{//\PYZlt{}/listing\PYZhy{}1\PYZgt{}}
      \PY{p}{\PYZob{}}
	\PY{k}{return} \PY{n}{p\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{*} \PY{n}{exp}\PY{p}{(}
	  \PY{p}{(}\PY{n}{l\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{+} \PY{p}{(}\PY{n}{c\PYZus{}pw}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{n}{c\PYZus{}pv}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{*} \PY{n}{T\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{/} \PY{n}{R\PYZus{}v}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{*} \PY{p}{(}\PY{k+kt}{real\PYZus{}t}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{/} \PY{n}{T\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{k+kt}{real\PYZus{}t}\PY{p}{(}\PY{l+m+mi}{1}\PY{p}{)} \PY{o}{/} \PY{n}{T}\PY{p}{)}
	  \PY{o}{\PYZhy{}} \PY{p}{(}\PY{n}{c\PYZus{}pw}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{n}{c\PYZus{}pv}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{/} \PY{n}{R\PYZus{}v}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{*} \PY{n}{std}\PY{o}{:}\PY{o}{:}\PY{n}{log}\PY{p}{(}\PY{n}{T} \PY{o}{/} \PY{n}{T\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)}
	\PY{p}{)}\PY{p}{;}
      \PY{p}{\PYZcb{}}

      \PY{c+c1}{// saturation vapour mixing ratio for water as a function of pressure and temperature}
      \PY{k}{template} \PY{o}{\PYZlt{}}\PY{k}{typename} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}
      \PY{n}{BOOST\PYZus{}GPU\PYZus{}ENABLED}
      \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{dimensionless}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{n}{r\PYZus{}vs}\PY{p}{(}
	\PY{k}{const} \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{temperature}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{o}{\PYZam{}}\PY{n}{T}\PY{p}{,}
	\PY{k}{const} \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{pressure}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{o}{\PYZam{}}\PY{n}{p}
      \PY{p}{)} \PY{p}{\PYZob{}}
	\PY{k}{return} \PY{n}{eps}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{/} \PY{p}{(}\PY{n}{p} \PY{o}{/} \PY{n}{p\PYZus{}vs}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{n}{T}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{l+m+mi}{1}\PY{p}{)}\PY{p}{;}
      \PY{p}{\PYZcb{}}

      \PY{c+c1}{// latent heat for constant c\PYZus{}p}
      \PY{k}{template} \PY{o}{\PYZlt{}}\PY{k}{typename} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}
      \PY{n}{BOOST\PYZus{}GPU\PYZus{}ENABLED}
      \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{divide\PYZus{}typeof\PYZus{}helper}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{energy}\PY{p}{,} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{mass}\PY{o}{\PYZgt{}}\PY{o}{:}\PY{o}{:}\PY{n}{type} \PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{n}{l\PYZus{}v}\PY{p}{(}
	\PY{k}{const} \PY{n}{quantity}\PY{o}{\PYZlt{}}\PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{temperature}\PY{p}{,} \PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}} \PY{o}{\PYZam{}}\PY{n}{T}
      \PY{p}{)} \PY{p}{\PYZob{}}
	\PY{k}{return} \PY{n}{l\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{+} \PY{p}{(}\PY{n}{c\PYZus{}pv}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)} \PY{o}{\PYZhy{}} \PY{n}{c\PYZus{}pw}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)} \PY{o}{*} \PY{p}{(}\PY{n}{T} \PY{o}{\PYZhy{}} \PY{n}{T\PYZus{}tri}\PY{o}{\PYZlt{}}\PY{k+kt}{real\PYZus{}t}\PY{o}{\PYZgt{}}\PY{p}{(}\PY{p}{)}\PY{p}{)}\PY{p}{;}
      \PY{p}{\PYZcb{}}
    \PY{p}{\PYZcb{}}\PY{p}{;}
  \PY{p}{\PYZcb{}}\PY{p}{;}
\PY{p}{\PYZcb{}}\PY{p}{;}
\end{Verbatim}


==> lst/pygments.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> lst/test_common_pvs.cpp.tex <==
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c+c1}{//\PYZlt{}listing\PYZhy{}1\PYZgt{}}
\PY{c+cp}{\PYZsh{}}\PY{c+cp}{include \PYZlt{}libcloudph++}\PY{c+cp}{/}\PY{c+cp}{common}\PY{c+cp}{/}\PY{c+cp}{const\PYZus{}cp.hpp\PYZgt{}}

\PY{k+kt}{int} \PY{n+nf}{main}\PY{p}{(}\PY{p}{)}
\PY{p}{\PYZob{}}
  \PY{k}{using} \PY{k}{namespace} \PY{n}{libcloudphxx}\PY{o}{:}\PY{o}{:}\PY{n}{common}\PY{o}{:}\PY{o}{:}\PY{n}{const\PYZus{}cp}\PY{p}{;}
  \PY{n}{assert}\PY{p}{(}\PY{n}{p\PYZus{}vs}\PY{p}{(}\PY{l+m+mf}{273.16} \PY{o}{*} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{kelvins}\PY{p}{)} \PY{o}{=}\PY{o}{=} \PY{l+m+mf}{611.73} \PY{o}{*} \PY{n}{si}\PY{o}{:}\PY{o}{:}\PY{n}{pascals}\PY{p}{)}\PY{p}{;}
\PY{p}{\PYZcb{}}
\PY{c+c1}{//\PYZlt{}/listing\PYZhy{}1\PYZgt{}}
\end{Verbatim}

